Fusing Reward and Dueling Feedback in Stochastic Bandits

This paper investigates the fusion of absolute (reward) and relative (dueling) feedback in stochastic bandits, where both feedback types are gathered in each decision round. We derive a regret lower bound, demonstrating that an efficient algorithm may incur only the smaller among the reward and dueling-based regret for each individual arm. We propose two fusion approaches: (1) a simple elimination fusion algorithm that leverages both feedback types to explore all arms and unifies collected information by sharing a common candidate arm set, and (2) a decomposition fusion algorithm that selects the more effective feedback to explore the corresponding arms and randomly assigns one feedback type for exploration and the other for exploitation in each round. The elimination fusion experiences a suboptimal multiplicative term of the number of arms in regret due to the intrinsic suboptimality of dueling elimination. In contrast, the decomposition fusion achieves regret matching the lower bound up to a constant under a common assumption. Extensive experiments confirm the efficacy of our algorithms and theoretical results.

==> sections/11_rebuttal_icml_25.tex <==
% !TeX root = ../dueling-reward-bandits.tex
\section{Detail Responses to ICML 2025}

% \subsection*{General global comment:}

\subsection{Reviewer 6nVK (Score 2 / Weak Reject)}

\begin{enumerate}
    \item[\check] \review{I feel that it is a bit overclaimed that "DecoFusion achieves the optimal regret". While the main theorem (Theorem 4.1) seems valid, the result is so asymptotic, that the optimality is not achieved as soon as the number of arms K is not constant (see W1)}
          \review{W1) In my view, the regret bounds are of high asymptotic nature. For instance, the regret bound in Theorem 4.1 only matches the lower bound only in the regime where \(T\geq \exp [ c K]\), which is quite disappointing.
          }
          \\
          \answer{
              We respectfully disagree with the reviewer's characterization of our results as "disappointing," particularly regarding the asymptotic nature of our bound matching.
              As detailed below, achieving asymptotic optimality in this context is a well-established practice in bandit literature.
              We hope the reviewer will reconsider the contributions of our paper in light of these points.
              \\
              % We respectfully disagree with the reviewer's characterization of our results as ``disappointing,'' as our upper bound is expected to match the lower bound in an asymptotic sense—a standard practice in bandit literature.
              % We respectively disagree with the reviewer that our results are ``disappointing'' for the fact that our upper bound only matches our lower bound in an asymptotic manner. 
              % As clarified below, 
              % this has been the standard practice in bandit literature from the very beginning.
              % Therefore, the comment from the reviewer is a bit unfair, and 
              % As clarified below, we sincerely hope the reviewer can re-evaluate the contributions of this paper.
              % \\
              Firstly, while our (gap-dependent) upper bound is non-asymptotic for any \(T\), it is expected to match the lower bound only in an asymptotic manner.
              Because the (gap-dependent) lower bounds in bandits literature (as well as our Theorem 3.1) are usually asymptotic (holds when \(T\to\infty\)), and thus the upper bounds can only match them in an asymptotic manner.
              This is a common practice for optimal bandit algorithms.
              For example, the regret upper bounds of the known optimal stochastic bandit algorithms, e.g., KL-UCB~\citep[Theorem 1]{cappe2013kullback} and DMED~\citep[Theorem 4]{honda2010asymptotically}, also match the lower bound only in an asymptotic manner.
              \\
              Secondly, the condition \(T\ge \exp(cK)\) for matching lower bounds is common and needed in most bandits algorithms (omitted by default, so this is often not aware).
              For example, the regret upper bound of the seminal UCB1 algorithm~\citep[Theorem 1]{auer2002finite} can be expressed as \[
                  R_T \le O\left( \sum_{k>1}\frac{\log T}{\Delta_k} + K \right).
              \]
              To match the \(\Omega\left( \sum_{k>1}\frac{\log T}{\Delta_k}\right)\) lower bound, it needs \(T \ge \exp (cK)\) as well.
              This condition is required for any bandit algorithm whose finite (gap-dependent) regret upper bound has an additive \(O(K)\) term---a very common term in the literature.
              Therefore, the required condition \(T\ge \exp(cK^{1+\xi})\) in our Theorem 4.1 is also standard as \(\xi\) can be as close to zero as possible.
          }


          %   \paragraph{Nudge AC:} Dear AC and SAC,
          %   \\
          %   As the discussion deadline is approaching and the reviewer does not explicit respond to our rebuttal, we would like to take the chance to summarize the key point of our rebuttal.

          %   Reviewer 6nVK raised a concern that our upper bound is disappointing because it only matches the lower bound in an asymptotic manner, and only when the condition \(T\ge \exp(cK)\) holds.

          %   Although both statements are true, we respectfully disagree with their ``disappointing'' characterization.
          %   Because  both statements are common practices in bandit literature.
          %   First, the asymptotic matching between (gap-dependent) upper and lower bounds is a standard practice in bandit literature.
          %   Since the standard (gap-dependent) lower bounds are asymptotic themselves, one can only expect the upper bounds to match them in an asymptotic manner.
          %   Second, the \(T\ge \exp(cK)\) condition is required in almost all (gap-dependent) regret upper bounds in bandits to match with lower bounds. On typical example is the seminal UCB1 algorithm in Auer et al. (2002) and its vast among of follow-ups. We explain this in detail in our A1 above.

          %   We also want to take the chance to thank the reviewers and area chairs for their time and effort in reviewing our paper. We are looking forward to your feedback on our rebuttal and the final decision.

          %   Best regards,
          %   Authors.


          \paragraph{Nudge AC:} Dear AC and SAC,
          As the discussion deadline approaches and Reviewer 6nVK did not explicitly reply to our rebuttal, we would like to take this opportunity to summarize its key points.

          Reviewer 6nVK noted that our upper bound is “disappointing” because it only matches the lower bound in an asymptotic sense and only under the condition \(T\ge \exp(cK)\). While these observations are factually correct, we respectfully disagree with the negative characterization. Both aspects are standard practice in the bandit literature.

          First, asymptotic matching between (gap-dependent) upper and lower bounds is common because the lower bounds themselves are asymptotic; therefore, one can only expect the upper bounds to match them in an asymptotic manner. Second, the requirement \(T\ge \exp(cK)\) appears in nearly all (gap-dependent) regret upper bounds in bandits to align with the lower bounds. A typical example is the seminal UCB1 algorithm presented in Auer et al. (2002) and its many subsequent developments, as we detail in our A1 response above.

          We also wish to thank the reviewers and area chairs for their time and effort in evaluating our paper. We look forward to your feedback on our rebuttal and the final decision.

          Best regards,
          Authors.

    \item[\check] \review{C1)
              \(\epsilon\) is not defined the statement of Theorem 4.1
          }
          \\
          \answer{
              We thank the reviewer for pointing this typo out.
              The \(\xi\) and \(\epsilon\) are the same in the statement of Theorem 4.1, and we will correct this in the final version.
          }


    \item[\check] \review{Q1) In Section 2, you write "Later in this paper, we will show that a sublogarithmic \(o(\log T )\) regret is actually achievable (in fact, T -independent constant regret) in these two scenarios, revealing a unique phenomenon of DR-MAB". Up to my knowledge, this phenomenon is not unique and in fact arises for bandit problems with side information (e.g. the player plays several arms and only incurs the regret of a single arm).}
          \\
          \answer{ We thank the reviewer for bringing up this line of works. We will add this line of reference in the final version of this paper.
              We will clarify also that the uniqueness of the phenomenon is in the context of the fusion of reward and dueling feedback, in comparison to the bandits with either reward or dueling feedback.
          }

    \item[\check] \review{Q2) Following W1, I am wondering to what extent using more recent approaches in duelling bandits allows to bypass the limitation that we need \(T\ge \exp\left( cK^{1+\xi} \right)\)
              for optimality.}
          \\
          \answer{Although there are indeed some recent progress on dueling bandits, e.g., the best-of-both world algorithm by~\citet[Theorem 3]{saha2022versatile} (whose stochastic regret upper bound has a suboptimal prefactor \(4\) in the dominating \(\log T\) term), to the knowledge of the authors, the best known regret bounds for stochastic dueling bandits is still the RMED algorithm by~\citet[Theorem 3]{komiyama2015regret}, which also relies on the \(T\ge \exp\left( cK^{1+\xi} \right)\) condition.
              We will add this discussion in the final version of this paper and raise this as an open question for future research in dueling bandits.
          }
\end{enumerate}


\subsection{Reviewer YVjo (Score 2 / Weak Reject)}

\begin{enumerate}
    \item[\check] \review{First, the practical value of the paper is not clear. The setting and framework are too simplistic and niche, making them inapplicable to motivating examples such as large language models (LLMs), which utilize inherently different algorithms and techniques.}
          \\
          \answer{
              \\
              While the authors agree that the bandits setting (a framework in favor of theoretical analysis) of this paper is indeed simplified, we believe that the proposed algorithms and theoretical results are still valuable for practice for the following reasons:
              \\
              The standard LLM training usually has two separate steps: (1) use the responses from human experts (absolute feedback)  to conduct a supervised learning, called supervised fine-tuning (SFT),
              and (2) use the human preference (relative feedback) among multiple responses generated from the SFT model to conduct a preference directly training (either directed preference optimization (DPO) or reinforcement learning from human feedback (RLHF)).
              \\
              %   \textbf{the following statement is not intact. Reconsider this answer.}
              Although not exactly the same, these two steps correspond to the reward (absolute) and dueling (relative) feedback in our bandits setting.
              Our algorithm suggests a training approach to conduct these two steps in parallel, which can potentially save the human labeling cost and improve the training efficiency (as our regret upper bounds improve over the existing ones). Investigating this potential approach in LLM training is an interesting direction.
              \\
              As our ultimate goal is to effectively combine the absolute and relative feedback (e.g., in realistic RLHF alignment for LLM), we believe that the proposed algorithms and theoretical results in the bandits framework are meaningful and concrete steps toward this goal.
              We thank the reviewer for raising this concern. We will add the discussion of this point in the final version of this paper.
          }
    \item[\check] \review{Second, the theoretical results appear to be a combination of existing tools and findings, which makes them somewhat expected. While the lower bound seems complete and logical, the algorithms do not appear to align with this lower bound. The only aspect that seems specific to this paper is the method of fusing these two feedback models and eliminating arms based on the best statistics (relative feedback or reward), which remains an open question. Specifically, the results align with the lower bound only when the best relative arm for eliminating a suboptimal arm is the one with the highest reward. This limitation also constrains the theoretical contribution, which seems to be the primary focus of the paper.
          }
          \\
          \answer{
              First, we clarify that our paper focuses on fusing both reward and dueling feedback, each drawn from distributions from a different set of parameters,
              and the information on neither type of feedback can not be translated into the other type.
              Due to this separation, it is intrinsically difficult to incorporate them to optimize performance on the same bandit task.
              To address the difficulty, we propose two novel algorithmic frameworks: elimination fusion and decomposition fusion, neither of which is known in prior literature.
              The elimination fusion is simple and more straightforward to be extended to other applications. In contrast, the decomposition fusion is optimized for the stochastic bandit scenario and achieves near-optimal regret performance.
              \\
              Secondly, we agree with the reviewer that
              removing the condition that ``the best relative arm for eliminating a suboptimal arm is the one with the highest reward'' (i.e., \(\ell_k^*=1\)) is indeed an interesting direction,
              as we discussed in the paper (Lines 382--384 (right column) and Lines 396--408 (left column)),
              However,
              this required condition is a reminiscence of the dueling bandits setting, and it is still a partially open problem~\citep{komiyama2015regret}.
              Once this problem is fully addressed in the basic dueling bandits, one can apply our two fusion algorithm techniques to the new dueling bandits algorithms to remove this condition in our setting.
          }
          % \xutong{Perhaps also mention our challenge of fusing the reward and dueling feedback.}
    \item[\check] \review{``The estimations of reward means \(\mu_k\)
              and dueling probabilities \(\nu_{k,\ell}\)
              are orthogonal as their observations are independently sampled from distributions with different parameters. This orthogonality makes it difficult to directly combine these two types of feedback in online learning.''
              \\
              The statement appears to be problematic. In what sense are these estimations considered orthogonal? Does "orthogonal" here imply independence? The reward feedback can clearly be translated into relative feedback, which suggests a relationship between the two types of feedback rather than a complete orthogonality. It may be beneficial to clarify this terminology to avoid confusion.
          }
          \\
          \answer{
              We thank the reviewer for suggesting the improvement of this phrase.
              Although there is indeed an ordering relation that ``the dueling probability of arm \(k\) winning over arm \(\ell\) is greater than \(0.5\) if and only if arm \(k\) has a higher expected reward than arm \(\ell\),''
              we clarify that the reward feedback cannot be directly translated into dueling feedback in the general case, unless some stronger relations are assumed between the reward means and dueling probabilities (e.g., the Bradley-Terry model suggested by Reviewer qwFm (hyperref)).
              \\
              In the final version of this paper, we will clarify the terminology and rewrite this sentence to avoid the confusion as follows,
              \\
              ``As the reward means and dueling probabilities only have a weak ordering relation---the dueling probability of arm \(k\) winning over arm \(\ell\) is greater than \(0.5\) if and only if arm \(k\) has a higher reward mean than arm \(\ell\)---and their observations are independently sampled from distributions with different parameters,
              the estimations of reward means \(\mu_k\)
              and dueling probabilities \(\nu_{k,\ell}\)
              are intrinsically separated.
              This separation makes it difficult to combine these two types of feedback in online learning directly.''
          }
\end{enumerate}


% \paragraph{Nudge AC:} Dear AC and SAC,
% \\
% As the discussion deadline is approaching and the reviewer does not explicit respond to our rebuttal, we would like to take the chance to summarize the key point of our rebuttal.

% Reviewer YVjo raised two key concerns on this paper: (1) the practical value, and (2) the theoretical novelty.


% For the practical value (details in A1), our fusing of reward and dueling feedback is a concrete step toward the ultimate goal of effectively combining absolute and relative feedback in realistic RLHF alignment for LLMs.

% For technique novelty (details in A2), this paper focuses on fusing the reward and dueling feedback, instead of addressing an open problem in dueling bandits (suggested by Reviewer YVjo).
% We propose two novel algorithmic frameworks: elimination fusion and decomposition fusion, neither of which is known in prior literature.
% The elimination fusion is by sharing the candidate arm sets of two elimination algorithms, and simple its idea has the potential to be extended for other applications.
% In contrast, the decomposition fusion is optimized for the stochastic bandit scenario and achieves near-optimal regret performance with three novel components (detailed in Section 4.2): decomposition arm set construction, randomized decision making, and exploration arm set construction. Its design challenges and high-level ideas are detailed in Section 4.1 in our paper.


% Best regards,
% Authors.


\paragraph{Nudge AC:} Dear AC and SAC,
As the discussion deadline approaches and Reviewer YVjo did not explicitly address our rebuttal, we would like to summarize the key points.

Reviewer YVjo raised two key concerns: (1) the practical value and (2) the theoretical novelty of our work.

For practical value (details in A1), our fusion of reward and dueling feedback is a concrete step toward effectively combining absolute and relative feedback in realistic RLHF alignment for LLMs. Our elimination and decomposition fusion techniques provide a fundamental insights for future empirical algorithm designs for LLM training, which is a promising research direction.

For theoretical novelty (details in A2), rather than addressing an open problem in dueling bandits as suggested, our focus is on fusing reward and dueling feedback through two novel algorithmic frameworks—elimination fusion and decomposition fusion—that are absent in prior literature. The elimination fusion approach shares candidate arm sets between two elimination algorithms, and the decomposition fusion, optimized for stochastic bandits, achieves near-optimal regret through three innovative components: decomposition arm set construction, randomized decision making, and exploration arm set construction (see Sections 4.1 and 4.2).

Best regards,
Authors.

\subsection{Reviewer TSNv (Score 4 / Accept)}

\begin{enumerate}
    \item[\check] \review{The regret bound for No Fusion algorithm seems to be different in the Table 1 and line 224 (right)}
          \\
          \answer{Indeed, they are different.
              The regret bound in Table 1 is the combination of two separate (optimal) regret bounds for the reward and dueling bandits, respectively. Therefore, the deminonator is \(\min\{(\Delta_k^{(R)})^2,\Delta_k^{(D)})^2 \}\) as both are in the best dependence.
              Nevertheless, the regret bound in line 224 is by combining two elimination algorithms for reward and dueling bandits, respectively (for the sake of comparison with our fusion elimination algorithm). As the elimination algorithm in dueling bandits is suboptimal, the denominator becomes  \(\min\{(\Delta_k^{(R)})^2,\Delta_k^{(D)})^2 / K \}\).
              \\
              We thank the reviewer for raising this concern. We will clarify this in the final version of this paper.
          }
    \item[\check] \review{The empirical log-likelihoods seems to be defined in algorithm 2, not algorithm 1 or 4.
          }
          \\
          \answer{
              Yes, it is the case because the empirical log-likelihoods are only used in Algorithm 2 (also updated in Algorithm 2 at Lines 29-30). Algorithms 1 and 4 do not need the empirical log-likelihoods.
          }
    \item[\check] \review{In the reward explore, dueling exploit stage, is there a reason to define the dueling action as both \(\hat k_t^R\)
          }
          \\
          \answer{
          Yes, as the arm \(\hat k_t^{(R)}\) is the current empirical best arm, we choose the empirical best arm pair \((\hat k_t^{(R)}, \hat k_t^{(R)})\) as the dueling action to exploit the empirical good arms (for the sake of minimizing the dueling regret since we only explore via reward feedback in that case).
          }


    \item[\check] \review{The algorithm line 6 and 8 does not do the exclusion of the reward set form dueling set as in line 264(right). Is there an intuition that this kind of non-approximate design works?}
          \\
          \answer{We thank the reviewer for catching this delicate but important algorithm design technique.
          \\
          In Line 264 (right), as the ground-truth decomposition is known, one should definitely exclude the reward set from the dueling set and vice versa.
          However, as the actual decomposition is unknown a prior in \defusion, we need to be conservative (i.e., allow both sets \(\hat{\mathcal K}_t^{(D)}\) and \(\hat{\mathcal K}_t^{(R)}\) to have some overlap instead of taking exclusion) to ensure enough explorations from both feedback sides for uncertain arms so to learn the ground-truth decomposition at the end.
          \\
          We will add this discussion in the final version of this paper to clarify the intuition behind this design.
          }
\end{enumerate}



\subsection{Reviewer qwFm (Score 4 / Accept)}

\begin{enumerate}
    \item[\check] \review{(Not a weakness, just a comment) In the formulation, this paper only considers that the preference probability of choosing arm a over arm b is greater than 0.5 if arm a has a higher expected reward than arm b. Besides this ordering relation, this paper does not assume or utilize any other relation between the preference probability and expected reward.
              What if the preference probability is generated according to the expected reward, like the Bradley-Terry model used in the RLHF literature? Will this additional assumption allow a better regret result? More discussion is needed here.}
          \\
          \answer{
              We thank the reviewer for raising this intriguing question.
              A relation between the preference probability and expected reward, like the Bradley-Terry model
              \(\nu_{1,2} = \frac{\exp(\mu_1)}{\exp(\mu_1) + \exp(\mu_2)} = \frac{\exp(\mu_1-\mu_2)}{\exp(\mu_1-\mu_2) + 1}\)
              or utility dueling bandits \(\nu_{1,2} = \frac{1 + (\mu_1 - \mu_2)}{2}\)~\citep{ailon2014reducing}, is indeed stronger than the one in our paper and will lead to a better regret result.
              \\
              Specifically, with this parametric relation, one only needs to focus on one set of the parameters, either the reward means or the dueling probabilities.
              Let us consider the case that the reward mean \((\mu_1, \mu_2, \dots, \mu_K)\) as the basic parameters to estimate, and all observations from dueling feedback can be translated into reward feedback via the parametric relation.
              Under this point of view, the reward feedback provides direct observations from the reward mean parameters,
              and the dueling (preference) feedback between arms \(k\) and \(\ell\) can be considered as a ``parametric reward feedback'' depending on the reward mean parameters.
              For example, with the Bradley-Terry relation, the parametric form is a logistic function, which is similar to the logistic bandits~\citep{faury2020improved}, while with the utility dueling relation,  the parametric form is a linear function, which is similar to the linear bandits~\citep{abbasi2011improved}.
              \\
              With this interpretation, the authors believe that the final regret bound would depend on reward gaps \(\Delta_k^{(R)}\) and have no explicit dependence on the dueling gaps \(\Delta_k^{(D)}\) (or the other way round if we consider the dueling probabilities as the basic parameters),
              and the regret improvement may be in the actual dependence of the reward gaps \(\Delta_k^{(R)}\) (e.g., the prefactor or the exponential order of this gap would be strictly less than than the best one without the dueling feedback option). To rigorously investigate the improvement in regret bounds under these stronger assumptions (out of the scope of current paper) is an interesting research direction.
              \\
              We will add this discussion in the final version of this paper to clarify the potential improvement in regret bounds under these stronger assumptions.
          }

    \item[\check] \review{What is the motivation of the regret definition (the equation above Section 2.1), which is a linear combination between the regret in classic bandits and the regret in dueling bandits? It seems that this is not very natural. Isn't it more natural to define the regret as the loss in the expected reward due to not always selecting the optimal arm, which may need an additional assumption that the preference probability is generated according to the expected reward, like the Bradley-Terry model?
          }
          \\
          \answer{
              We thank the reviewer again for raising this interesting question.
              \\
              \textbf{Motivation} The current linear combination defintion--- especially, the parameter \(\alpha\in[0,1]\)---is motivated by the cost difference between querying a reward feedback, as a dueling feedback, as the dueling (relative) feedback is usually cost-efficient~\citep{ouyang2022training}.
              Furthermore, this flexible definition covers many interesting scenarios, e.g., the case of \(\alpha = 1\) is the regret from reward feedback only, and the case of \(\alpha = 0\) is the regret from dueling feedback only,
              and in the case of \(\alpha = \frac{1}{2}\), the regret is the simple sum of the two types of feedback.
              We will add this discussion in the final version of this paper to clarify the motivation of the regret definition.
              \\
              Below, we provide three perspectives on changing the definition of regret in our paper.
              \\
              First, if the reviewer means to only consider the regret from reward feedback (``define the regret as the loss in the expected reward''), and treat the dueling feedback as a side free observations, then this regret reduces to the case of setting \(\alpha = 1\) in our regret definition.
              In this scenario, our \defusion algorithm achieves constant regret, as discussed in Lines 409--423 (left column).
              \\
              Second, if the reviewer means to also consider the regret cost due to dueling feedback but count this part of the regret in terms of the expected regret instead of the dueling (preference) probability in the current definition, then the new regret cost in each decision round would be the sum of the reward gaps of the pulled three arms (one for reward, a pair for dueling). For this new regret definition, our algorithm and analysis still works, and the only modification is in the regret upper bound results, where one needs to change the dueling gap \(\Delta_k^{(D)}\) in the nominator of Eq. (4) in Theorem 3.1 and Eq. (5) in Theorem 4.1 to the reward gap \(2\Delta_k^{(R)}\).
              \\
              Third, if one further assumes the Bradley-Terry model relation between reward means and dueling probabilities upon the new regret definition, this would lead to a problem that is similar to logistic bandits~\citep{faury2020improved}, as discussed in the previous response, which is an interesting research direction.
          }


\end{enumerate}
